Knot theory of complex plane curves

The primary objects of study in the ``knot theory of complex plane curves'' are C-links: links (or knots) cut out of a 3-sphere in the complex plane by complex plane transverse and totally tangential. Transverse C-links are naturally oriented. There are many natural classes of examples: links of singularities; links at infinity; links of divides, free divides, tree divides, and graph divides; and--most generally--quasipositive links. Totally tangential C-links are unoriented but naturally framed; they turn out to be precisely the real-analytic Legendrian links, and can profitably be investigated in terms of certain closely associated transverse C-links. The knot theory of complex plane curves is attractive not only for its own internal results, but also for its intriguing relationships and interesting contributions elsewhere in mathematics. Within low-dimensional topology, related subjects include braids, concordance, polynomial invariants, contact geometry, fibered links and open books, and Lefschetz pencils. Within low-dimensional algebraic and analytic geometry, related subjects include embeddings and injections of the complex line in the complex plane, line arrangements, Stein surfaces, and Hilbert's 16th problem.

==> coverpg.tex <==
\begingroup
\vspace*{42pt}
\centering
{\large\textbf{Table of Contents for the Handbook of Knot Theory}}

\smallskip

{William W. Menasco and Morwen B. Thistlethwaite, Editors}

\vspace*{36pt}

\begin{enumerate}
\addtolength{\itemsep}{12pt}
%
%
\item Colin Adams, 
\href{http://arxiv.org/abs/math.GT/0309466}{\textit{Hyperbolic knots}}
%
%
\item Joan S. Birman and Tara Brendle, 
\href{http://arxiv.org/abs/math.GT/0409205}{\textit{Braids: a survey}}
%
\item John Etnyre, 
\href{http://arxiv.org/abs/math.SG/0306256}%
{\textit{Legendrian and transversal knots}}
%
%
\item Greg Friedman,
\href{http://arxiv.org/abs/math.GT/0410606}%
{\textit{Knot spinning}}
%
\item Jim Hoste, \textit{The enumeration and classification 
of knots and links}
%
%
\item Louis Kauffman, 
\href{http://arxiv.org/abs/math.GT/0410329}{
\textit{Knot Diagrammatics}}
%
%
\item Charles Livingston, 
\href{http://arxiv.org/abs/math.GT/0307077}%
{\textit{A survey of classical knot concordance}}
%
%
\item Lee Rudolph, 
\href{http://arxiv.org/abs/math.GT/0411115}%
{\textit{Knot theory of complex plane curves}}
%
%
\item Marty Scharlemann, 
\href{http://arxiv.org/abs/math.GT/0308155}%
{\textit{Thin position in the theory of classical knots}}
%
\item Jeff Weeks, 
\href{http://arxiv.org/abs/math.GT/0309407}%
{\textit{Computation of hyperbolic structures in knot theory}}
\end{enumerate}

\endgroup
\vfill


==> fiddles.tex <==
%% just a few fiddles with amsmath.sty:

\makeatletter
%%for use in tags of displayed equations, to avoid I and O (look like numerals)
\def\AlphSkipI#1{\expandafter\@AlphSkipI\csname c@#1\endcsname}
\def\@AlphSkipI#1{%
  \ifcase#1\or A\or B\or C\or D\or E\or F\or G\or H\or J\or
   K\or L\or M\or N\or P\or Q\or R\or S\or T\or U\or V\or W\or X\or
    Y\or Z\or AA\or BB\or CC\or DD \or EE\or FF\or GG\or HH\or JJ\or
   KK\or LL\or MM\or NN\or PP\or QQ\or RR\or SS\or TT\or UU\or VV\or 
   WW\or XX\or YY\or ZZ\else\@ctrerr\fi}
\renewcommand\theequation{\AlphSkipI{equation}}
\renewcommand\tagform@[1]{\maketag@@@{\textup{\ignorespaces%
(\textbf{#1})\unskip\@@italiccorr}}}
\makeatother
\renewcommand\ref[1]{\textup{\ref{#1}}} % 
\renewcommand\eqref[1]{\textup{\textbf{\ref{#1}}}} % 
\newcommand\dispeqref[1]{\textup{(\textbf{\ref{#1}})}} % 

%% assorted fiddles with elsart.cls:

\def\theenumii{\textup{\alph{enumii}}}


%% include index of definitions

\input{indexdef.tex}

\makeatletter

%% fiddle with table of contents indentation and depth:
\renewcommand*\l@section{\@dottedtocline{1}{0.0em}{1.3em}}
\renewcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.2em}}
\renewcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.1em}}
\def\tableofcontents{%
  \begin{small}
  \leftline {{\bfseries \contentsname\/}}
  \setcounter{secnumdepth}{6}%
% \setcounter{tocdepth}{2}% for final version
  \setcounter{tocdepth}{3}% for final version
  {\@starttoc{toc}}%
\end{small}
}

%% ditto for list of figures:
\def\listoffigures{%
  \begin{small}
  \leftline {{\bfseries \listfigurename\/}}
  {\@starttoc{lof}}%
\end{small}
}

%% to get around Elsevier copyright stuff, for the arXiv version only:
\def\ps@copyright{\let\@mkboth\@gobbletwo
  \def\@oddhead{}%
  \let\@evenhead\@oddhead
  \def\@oddfoot{%
    \def\@tempa{0}
    \ifx\@volume\@tempa
    {\hfil {\rmfamily\thepage} \hfil}
    \else
    \fi}%
  \let\@evenfoot\@oddfoot
}

%% to include the cover page, for the arXiv only:
\def\title@fmt#1#2{%
\input{coverpg.tex}%    added  
\newpage

\@ifundefined{@runtitle}{\global\def\@runtitle{#1}}{}%
\vspace*{12pt}             % Vertical space above title
  {\@titlesize #1\,\hbox{$^{#2}$}\par}%
  \vskip\@undertitleskip
\vskip24\p@  % Vertical space below title
  }

%%%
\setcounter{page}{0}\def\thepage{}
\iffalse
\fi

\makeatother



==> indexdef.tex <==
\makeatletter
\newif\if@restonecol
\def\theindex{\@restonecoltrue\if@twocolumn\@restonecolfalse\fi
  \columnseprule\z@ \columnsep 35\p@
  \twocolumn[\@xp\section\@xp*\@xp{\indexname}]%
  \thispagestyle{plain}%
  \let\item\@idxitem
  \parindent\z@  \parskip\z@\@plus.3\p@\relax
  \footnotesize}
\def\@idxitem{\par\hangindent 2em}
\def\subitem{\par\hangindent 2em\hspace*{1em}}
\def\subsubitem{\par\hangindent 3em\hspace*{2em}}
\def\endtheindex{\if@restonecol\onecolumn\else\clearpage\fi}
\def\indexspace{\par\bigskip}
\makeindex
\makeatother


==> mdefs.tex <==
\def\Figref#1{\mbox{Figure \textup{\ref{#1}}}}
\def\Secref#1{\S\ref{#1}}
\makeatletter
%% the following code for prescripts was written by Michael J. Downes
\DeclareRobustCommand{\prescript}[3]{%
  \@mathmeasure\z@\scriptstyle{#1}%  put the sup in box 0
  \@mathmeasure\tw@\scriptstyle{#2}% put the sub in box 2
  \ifdim\wd\tw@>\wd\z@
    \setbox\z@\hbox to\wd\tw@{\hfil\unhbox\z@}%
  \else
    \setbox\tw@\hbox to\wd\z@{\hfil\unhbox\tw@}%
  \fi
  % Do not let a preceding mathord symbol approach without any
  % intervening space.
  \mathop{}%
  % Use \mathopen to suppress space between the prescripts and the
  % base object even when the latter is not of type ord.
  \mathopen{\vphantom{#3}}^{\box\z@}_{\box\tw@}%
  #3%
}
\makeatother

%% for use in `calculus of bands' in braid groups: 
\newcommand\SideSet[2]{\prescript{#1}{}{#2}}





%%%% Greek:
\renewcommand\a{\alpha}
\renewcommand\b{\beta} 
\renewcommand\e{\epsilon} 
\newcommand\g{\gamma} 
\renewcommand\d{\delta} 
\renewcommand\phi{\varphi} 
\newcommand\s{\sigma} 
\renewcommand\t{\tau}
\newcommand\x{\xi}
\newcommand\D{\Delta} 
\newcommand\G{\Gamma}

%%%% miscellany:

\newcommand\absband[1]{|{#1}|} % ``absolute value'' of a band
\newcommand\AKn[2]{A({#1},{#2})}  % annulus of type #1 with #2 twists
     \newcommand{\Akn}{\AKn{K}{n}}
     \def\AKN#1{A(K_#1,n_#1)} \def\AON#1{A(O_#1,n_#1)} % more of the same 
\newcommand{\after}{\mathop{\circ}} % composition
\newcommand\Alex[1]{\Delta_{#1}} % Alexander polynomial of #1
\renewcommand\arg[1]{\operatorname{arg}({#1})} % 
\newcommand\argument[1]{#1/|#1|}% argument of #1
\newcommand\As{\mathscr A}
\newcommand{\askfont}{\relax} % could be \textbf, etc.
\newcommand{\ask}[1]{\askfont{#1}} % for research questions
\newcommand\attach[1]{A({#1})}% attaching region of #1
\newcommand\Aut{\operatorname{Aut}} % automorphism group

\newcommand\basept{\ast} % basepoint
\newcommand\Bd{\partial} 
\newcommand\bhat{\widehat{b}} 
\newcommand\bi[1]{\operatorname{brin}({#1})} % braid index of #1
\newcommand\binding[1]{\mathbf{#1}^{-1}(0)} % binding of open book named #1
\renewcommand\bot{\operatorname{bot}} % bottom (of a Seifert surface)
\newcommand\bow[1]{{\bowtie_{#1}}}% bowtie
\newcommand\braidof[1]{\beta({#1})} % braid of (band rep. or braidword) #1 
\newcommand\brdiagram[1]{\mathbf{BD}({#1})}% braid diagram of #1
\newcommand\brep[1]{\mathbf{#1}} % band representation named #1 
\newcommand\brepvec[2]{\parentuple{#1}1{#2}} % ditto, as a vector
\newcommand\brinj[1]{\mathfrak{i}_{#1}} % canonical braidgroup injection
\newcommand\brgen[1]{\sigma_{#1}} % braidgroup generator with index #1
\newcommand\brgp[1]{B_{{#1}}} % braidgroup with basepoint #1
\newcommand\bSeif[1]{S[#1]} % braided Seifert surface with data #1
\newcommand\bStein{\mathbf{B}} % Stein ball
\newcommand\bsurf[1]{S({#1})} % braided surface of brep or bword named #1
\newcommand\bundlemap[1]{\xrightarrow{#1}} % bundle map named #1
\newcommand\bword[1]{\mathbf{#1}} % braidword or bandword named #1
\newcommand\bydeffont{\textsl} % could be \emph, or \textit, etc., etc.:
\newcommand\bydeffontname{slanted} % modify this accordingly 
%%%%%

%\makeatletter
%\newcommand\bydef[1]{\bydeffont\@ifnextchar k{{#1}\index Z@{#1}}{{#1}\index{#1}}}
%\makeatother
\newcommand\bydef[1]{\bydeffont{#1}\index{#1}}%
   \newcommand\moredef[1]{\bydeffont{#1}} % for (unindexed) continued defs

\newcommand\card[1]{\operatorname{card}({#1})} % cardinality of #1
\newcommand\C{\mathbb C} % complex numbers
\newcommand\Cext{\P_1(\C)} %% Riemann sphere (extended complex numbers)
\newcommand\CH[2]{H^{\scriptscriptstyle({#1})}_{#2}} % coarse handle of index #1
\newcommand\charfun[1]{c_{\scriptscriptstyle{#1}}} % (multi)characteristic function of #1
\DeclareMathSymbol{\circmapsymbol}{\mathord}{AMSa}{"09}
\newcommand\circmap[1]{\circmapsymbol^{#1}}% homotopy class of z^#1
\newcommand\clasp[1]{\operatorname{clasp}({#1})} % clasp number of #1
\newcommand\Clink{$\C$\nobreakdash-} % 
\newcommand\clint[2]{\mbox{$[#1,#2]$}} % closed interval from #1 to #2
\newcommand\clopint[2]{\mbox{$[#1,#2{[}$}} % right-half-open interval (Bourbaki style)
\newcommand\closedbraid[1]{{\widehat\beta}({#1})} % closed braid of #1
\newcommand{\col}[2]{\operatorname {col}_{#1\subset #2}}% collaring (map)
\newcommand{\collar}[2]{\operatorname{Col}({#1}\sub{#2})}% collar (subspace)
\newcommand\concat{\smallfrown} % concatenation
\newcommand\config[1]{\subsets{#1}{\C}} % #1th configuration space C
%%making complex conjugation attractive:
\makeatletter
\DeclareRobustCommand{\c@njug}[1]{
   #1\setbox0=\hbox{$#1$}\kern-\wd0%
   \dimen1=\wd0\advance\dimen1 by -.15em
   \kern .1em \overline{\hbox to \dimen1{\hss\vphantom{$#1$}\hss}}\kern .05em%
}
\DeclareRobustCommand{\conjug}[1]{\c@njug{{{\mbox{$#1$}}}}}
\makeatother
%%%
\newcommand\conjugate[2]{\SideSet{#1}{#2}} % conjugate #2 by #1
\newcommand\cont[1]{C({#1})} % continuous functions from #1 to C
\newcommand\core[1]{\kappa({#1})} % core arc of a 1-handle 
\newcommand\corners{\mathsf{k}} % corners of a manifold
\newcommand\covmap[1]{{\xi}_{#1}} % covering map corresponding to rep'n #1
   \newcommand\brcovmap[1]{{\widetilde\xi}_{#1}} % branched covering ditto
\newcommand\cover[1]{\Xi_{#1}}% covering space corresponding to rep'n #1
   \newcommand\brcover[1]{{\widetilde{\Xi}}_{#1}} % branched covering space ditto
\newcommand\critpts[1]{\operatorname{crit}({#1})}% critical points of #1
\newcommand\critvals[1]{#1(\critpts{#1})}% critical values of #1
\newcommand\crossings[1]{\operatorname{cross}({#1})}% crossing number of #1
%\newcommand\commute[2]{\left[#1,#2\right]} % commutator %%% UGGLY
\newcommand\commute[2]{[{#1},{#2}]} % commutator 
\newcommand\compsof[1]{\pi_0({#1})} % set of components of #1 
\newcommand\Cs{\mathscr C}
\newcommand\cut[2]{{#1}\wr{#2}} % #1 ``cut open along'' #2 
\newcommand\cycle[1]{({#1})}

\newcommand\defines{\mathrel{=:}}% left side defines right side
\newcommand\degr[1]{\operatorname{deg}({#1})} % degree of f
\newcommand\den[1]{\operatorname{den}({#1})}% denominator of #1
\newcommand\derbun[1]{D#1} % derivative of #1 on bundle level
\newcommand\deriv[2]{D#1({#2})} % derivative of #1 at #2
\newcommand\dfuns[2]{\operatorname{Diff}({#1},{#2})}% smooth maps from #1 to #2
\newcommand\diagram[1]{\mathbf{D}({#1})}% diagram of #1
\newcommand\diff[2]{\hbox{${#1}\setminus{#2}$}} % difference of sets
\newcommand\divisor[1]{\mathbb{D}({#1})} % could be simply D({#1})
\newcommand\disc[2]{\Delta_#1({#2})} % #1th discriminant of #2
\newcommand\Disc[1]{\Delta({#1})} % discriminant of #1
%\newcommand\doublepts[1]{\operatorname{double}({#1})}% doublepoints of #1
\newcommand\doublepts[1]{\operatorname{doub}({#1})}% shorter version
\newcommand\dual[1]{[#1]^*}% dual (homology class) of #1

\newcommand\edgeband[1]{\mathsf{e}({#1})} % edge-class of a band
\newcommand\eedge{\mathbf e}
    \newcommand\fedge{\mathbf f}
    \newcommand\gedge{\mathbf g} % edges
\newcommand{\emband}[2]{\sigma_{{\scriptscriptstyle{#1,\mkern3mu #2}}}}
\renewcommand\emptyset{\varnothing} % purely a matter of taste
\newcommand\encloses{\Supset}
\newcommand\Ext[2]{\operatorname{Ext}({#1}\sub {#2})}% exterior of #1 in #2
\newcommand\ext{\operatorname{ext}} % extremum
\newcommand\Edges[1]{{\mathsf{E}}({#1})} % edges of #1
\newcommand\embto{\hookrightarrow}% embedding 
\newcommand\euler[1]{\chi({#1})}%cf. \genus
\newcommand\eulermax[2]{X_{#1}({#2})}%cf. \genus

\newcommand\F{\mathbb{F}} % ground field
\newcommand\fence{\mathsc{F}} % fence
\newcommand\Finf[1]{F_\infty({#1})}
\newcommand\foreignfont{\emph} % could be \textit, or \textsl, etc., etc.
\newcommand\foreign[1]{\foreignfont{#1}}
\newcommand\frdiagram[1]{\mathbf{FD}({#1})}% front diagram of #1
\newcommand\freegen[1]{{\mathbf{g}}_{{#1}}}% #1th free generator of a free group
\newcommand\freeprod{\ast}% free product
\newcommand\from{\colon\thinspace} %% 
\newcommand\fundgp[2]{\pi_1({#1};{#2})}% fundamental group of #1 based at #2
\newcommand\fundgpnbp[1]{\pi_1({#1})}% fundamental group of #1, no basepoint

\newcommand\gbraid[1]{{\gamma}({#1})} % geometric braid of #1
\newcommand\GCD{\operatorname{GCD}} 
\newcommand\genby[2]{\langle{#1}\rangle_{#2}}% subobject of #2 generated by #1 
\newcommand\genbyelt[2]{\langle{#1}\rangle_{#2}}% ditto, for single element #1
\newcommand\genus[2]{g_{#1}({#2})}% type-#1 genus of #2 (for ordinary, #1={})
\newcommand\geomrel[1]{\overstrike{|}{\|}{#1}\overstrike{\|}{|}}% geometric realization of #1
\newcommand\gp[2]{\operatorname{gp}
      \big({#1}\colon{#2}\big)} % group presentation
\newcommand\gr[1]{\operatorname{gr}({#1})} % (multi)graph of #1

\renewcommand\H[1]{\Hs({#1})}
\newcommand\Hs{\mathscr H}
\newcommand\h[2]{h^{\scriptscriptstyle({#1})}_{#2}} % handle of index #1
\newcommand\holo[1]{\mathscr{O}({#1})}% holomorphic functions/germs on #1
    \newcommand\nzholo[1]{\mathscr{U}({#1})}% nowhere-zero " "
    \newcommand\nizholo[1]{\mathscr{W}({#1})}% no interior zeros " " 
    \newcommand\intholo[1]{\mathscr{A}({#1})}% continuous on #1, holo on Int#1
\newcommand\holon[1]{{\prescript{}{#1}{\holo{}}}_{\zero}}%h-germs at 0 in C^#1
\newcommand\homcls[1]{[{#1}]} % homotopy class of #1 
\newcommand\hparam[1]{\eta_{\thinspace{#1}}} % handle parametrization
\newcommand\hunknot{\mathbb{O}'} % the horizontal unknot

\newcommand\inclusion[2]{\operatorname{i}_{{#1}\hookrightarrow{#2}}}%inclusion
\newcommand\id[1]{\operatorname{id}_{#1}} % identity map of #1
\renewcommand\Im{\operatorname{Im}} % imaginary part
\newcommand\imunit{i}% could be \mathrm{i} or \sqrt{-1}, per publisher's policy
\newcommand\imto{\looparrowright}% immersion 
\newcommand\ind[2]{\operatorname{ind}({#1};{#2})} % index of #1 at #2
\newcommand\info[1]{\mathbf{I}(\diagram{#1})} % information about #1
   \newcommand\brinfo[1]{\mathbf{I}(\brdiagram{#1})} % information about #1
   \newcommand\frinfo[1]{\mathbf{I}(\frdiagram{#1})} % information about #1
\newcommand\injection{\rightarrowtail}
\newcommand\inside[1]{\iota({#1})} % inside of #1 (a simple closed curve in \C)
\newcommand\Int[1]{\operatorname{Int}{#1}} % interior 
\newcommand\into{\hookrightarrow}% inclusion map of a subset
\newcommand\intsto[1]{\mathbf{#1}} % set of nonnegative integers less than %1
\DeclareRobustCommand{\inverse}[1]{\conjug{{{\mbox{$#1\vphantom{h}$}}}}}% inverse (narrow)
\newcommand\Is{\mathscr I}
\newcommand\isdefinedas{\mathrel{:=}}% right side defines left side
\newcommand\isosymbol{\cong} % symbol for natural isomorphism
\newcommand\iso{\linebreak[2]\isosymbol\linebreak[3]} % 

\newcommand\Kinf[1]{K_\infty({#1})} % knot at infinity of #1
\newcommand\knot[2]{#1_{\scriptscriptstyle{#2}}}
\newcommand\Kscr{\mathscr{K}}


\newcommand\Legf[1]{f^{\mathscr{L}}_{#1}}% Legendrian framing of #1
\newcommand\liftof[1]{\widetilde#1} % ``lift'' of #1
\newcommand\link[2]{\operatorname{link}({#1},{#2})}%linking of #1 and #2
\newcommand\Lscr{\mathscr{L}}
\newcommand\length{\ell}
\newcommand\LHP{\C_{-}} % (closed) lower half-plane
    \newcommand\UHP{\C_{+}} % (closed) upper half-plane
    \newcommand\EHP{\C_{\pm}} % either (closed) half-plane

\newcommand\merid[2]{\mathord{\pitchfork}({#1};{#2})}% 
   \newcommand\Bdmerid[2]{\Bd\thinspace\mathord{\pitchfork}({#1};{#2})}% 
\newcommand\mero[1]{\mathscr{M}_{#1}}% meromorphic functions/germs on #1
\newcommand\meron[1]{{\prescript{}{#1}{\mero{}}}_{\zero}}%h-germs at 0 in C^#1
\newcommand\meromapto{\dashrightarrow}%% rational or meromorphic map
%%% Apparently some laser printers (mine!) won't print \dashrightarrow !!! so:
\renewcommand\meromapto{\rightsquigarrow}

\newcommand\Mgood{\mbox{M-M--good}} % "Milnor-Morse good"
\newcommand\Milnorfiber[1]{F_{#1}}% Milnor fiber of #1
\newcommand\Milnornumber[1]{\mu({#1})}% Milnor number of #1
\newcommand{\Mir}{\operatorname {Mir}} % mirror image
\newcommand\Mmap[1]{\phi_{#1}} % Milnor map of #1 (at radius 1)
\newcommand\Mmapr[2]{\phi_{#1,#2}} % Milnor map of #1 at radius #2
\newcommand\MN{\mathscr{MN}} % Morse-Novikov number
\newcommand\modqp[1]{q({#1})}% modulus of quasipositivity of %1
\newcommand\monicpoly[1]{MP_{#1}} % affine space of monic poly's of degree #1
\newcommand\monogen[1]{{\mathsf{g}}_{{#1}}}% #1th generator of monodromy group
\newcommand\mult[1]{\mathbf{m}_{#1}} % multiplicity assigned to #1
\newcommand\multilink[2]{(#1,\mathbf{#2})}% multilink (support #1, mult.#2)
\newcommand\multiplepts[1]{\operatorname{mult}({#1})}% multiplepoints of #1
\newcommand\multito[1]{\overset{1:#1\thinspace}{\DOTSB\relbar\joinrel\multimap}}% another version
\newcommand\multpower[1]{\mathscr{MP}({#1})} % all multisubsets of #1
\newcommand\multsets[2]{{\mathscr{MP}^{[#2]}}({#1})} % #2-multisubsets of #1 
\newcommand\nbrid[1]{\ifx0#1{o}\else{o^{({#1})}}\fi} % identity of B_#1
\newcommand\nband[1]{${#1}$\nobreakdash-{}band} % 
	  \newcommand\nbraid[1]{${#1}$\nobreakdash-{}braid} % 
      \newcommand\ncell[1]{${#1}$\nobreakdash-cell}
      \newcommand\ncodimension[1]{codimension\nobreakdash-${#1}$}
      \newcommand\ncomponent[1]{${#1}$\nobreakdash-component}
      \newcommand\ndimensional[1]{${#1}$\nobreakdash-dimensional}
	  \newcommand\nstring[1]{${#1}$\nobreakdash-{}string} % 
      \newcommand\ntuple[1]{${#1}$\nobreakdash-tuple}
   \newcommand\nhandledash{\nobreakdash-} % could be \nobreakdash--
       \newcommand\ncycle[1]{${#1}$\nhandledash{}cycle} % 
       \newcommand\nhandle[1]{${#1}$\nhandledash{}handle} % 
       \newcommand\nstar[1]{${#1}$\nhandledash{}star} 
       \newcommand\ngon[1]{${#1}$\nhandledash{}gon} 
       \newcommand\nsubset[1]{${#1}$\nhandledash{}subset} 
   \newcommand\nmanifolddash{\nobreakdash--} % could be \nobreakdash-
       \newcommand\ndisk[1]{${#1}$\nmanifolddash{}disk} 
       \newcommand\nsphere[1]{${#1}$\nmanifolddash{}sphere} 
       \newcommand\nmanifold[1]{${#1}$\nmanifolddash{}manifold} 
       \newcommand\nsubmanifold[1]{${#1}$\nmanifolddash{}submanifold} 
\newcommand\naive{na{\"\i}ve}% could be without diaresis if publisher insists
\newcommand\naively{{\naive}ly}% consistent with above
\newcommand\N{\mathbb N} 
\newcommand\Nstrict{\N_{>0}} 
\newcommand\Nb[2]{\operatorname{Nb}({#1}\sub{#2})}%regular nbhd of #1 in #2
\newcommand\nmultpower[2]{\mathscr{MP}^{[#1]}({#2})} % #1-element multisubsets of #2
\newcommand\node[1]{\operatorname{node}({#1})} % node number of #1
\newcommand\noknot{{\displaystyle{\varnothing}}}%%      
\newcommand\norm[1]{\|#1\|} 
\newcommand\normbun[1]{\nu({#1})} % total space of the normal bundle of #1
\newcommand\npower[2]{\mathscr{P}^{[#1]}({#2})} % #1-element subsets of #2
\newcommand\nstratum[2]{({#2})^{[#1]}} % stratum of #2 of type #1
\newcommand\num[1]{\operatorname{num}({#1})}% numerator of #1
\newcommand\numk{\intsto{k}}
\newcommand\numn{\intsto{n}}

\newcommand\ob[1]{\mathbf{#1}} % open book named #1
\newcommand\of[1]{({#1})}%as in, "FUNCTION of ARGUMENT"; helps paren matching
\newcommand\ontuple[2]{\tuple{#1}{1}{#2}}% ordered #2-tuple of #1s
\newcommand\Os{\mathscr O}
\newcommand\ogonek%
  {\kern-.45em\lower.72ex\hbox{$\scriptstyle\mathchar'454$}\kern.25em}
\newcommand\opint[2]{\mbox{${]}#1,#2{[}$}} % open interval from #1 to #2 (Bourbaki)
\newcommand\opclint[2]{\mbox{${]}#1,#2]$}} % left-half-open interval (Bourbaki style)
\newcommand\ord{\operatorname{ord}} 
\newcommand\overarc[2]{\operatorname{over}_{#1}({\diagram{#2}})} % over-arc of #2 at #1
\newcommand\overx[1]{{#1}^{\smallsmile}}%overcrossing at #1

\renewcommand\P{\mathbb P} 
\newcommand\page[2]{S({#1},{#2})}% page of Morse map #1 with argument #2
\newcommand\partition[1]{\mathbf{#1}} % a partition named #1
\newcommand\perm[1]{{\mathsf{#1}}} % a permutation named #1
\newcommand\phold{{\textstyle{\cdot}}}% placeholder; could be \cdot or - or \Box or ...
\newcommand\pict[1]{\mathbf{P}(\diagram{#1})} % picture of #1
   \newcommand\brpict[1]{\mathbf{P}(\brdiagram{#1})} % picture of #1
   \newcommand\frpict[1]{\mathbf{P}(\frdiagram{#1})} % picture of #1
\newcommand\posts[1]{\mathsf{P}({#1})} % posts of #1
\newcommand\power[1]{\mathscr{P}({#1})} % powerset of #1
\newcommand\pr{\operatorname{pr}}
\newcommand\pretzel[1]{\mathfrak{P}({#1})}% braidzel surface with data #1
\newcommand\proj[1]{\mathbf{p}_{\scriptscriptstyle\,\diagram{#1}}}% projection of the diagram of #1
\renewcommand\Pr{\eusm P} 
\newcommand\Ps{\mathscr{P}}
\newcommand\pushoff[1]{#1^{+}}

\newcommand\Q{\mathbb Q}

\newcommand\R{\mathbb{R}}
   \newcommand{\Rg}[1]{\R_{>{#1}}}
   \newcommand{\Rge}[1]{\R_{\ge{#1}}}
   \newcommand{\Rl}[1]{\R_{<{#1}}}
   \newcommand{\Rle}[1]{\R_{\le{#1}}}
   \newcommand\Rnonneg{\Rge{0}}
   \newcommand\Rpos{\Rg{0}}
   \newcommand\Rnonpos{\Rle{0}}
   \newcommand\Rneg{\Rl{<0}}
\newcommand\Rs{\mathscr{R}} 
\newcommand\rank{\operatorname{rank}}
\renewcommand\Re{\operatorname{Re}} % real part
\newcommand\reduced[1]{\widetilde#1} % reduced (homology group)
\newcommand\reg[1]{\operatorname{Reg}({#1})} % regular points of #1
\newcommand\regkth[2]{\operatorname{Reg}^{#1}({#2})} 
\newcommand\relator[1]{{\mathbf{r}}_{{#1}}}% #1th relator
\newcommand\repn[1]{\rho_{#1}}% representation
\newcommand\resolve{R}% resolution map
\newcommand\resp[1]{{\textup(}resp., #1\textup{)}} % respectively, #1
\newcommand\restr{{\mathrel |}} % restriction (of a map)
\newcommand{\roots}{r}% ``roots'' map

\newcommand\Ss{\mathscr S} 
\newcommand\scbc[1]{\mathsf{C}_{#1}}% standard cyclic branched cover of degree #1 
\newcommand*\see[2]{\textit{see} #1}
\newcommand\Seifmatrix[1]{[#1]} % Seifert matrix 
\newcommand\Seifo{{\mathord{\mathsf{o}}}} % Seifert circle
\newcommand\Seifx{{\mathord{\mathsf{x}}}}% (Seifert) crossing
\newcommand\Seify{{\mathord{\mathsf{y}}}}% a second (Seifert) crossing
\newcommand\Seifz{{\mathord{\mathsf{z}}}}% a third (Seifert) crossing
\newcommand\SeifO[1]{\mathord{\mathsf{O}}_{#1}} % Seifert circles
\newcommand\SeifX[1]{\mathord{\mathsf{X}}_{#1}}% (Seifert) crossings
\newcommand\Seifframe[2]{f_{{#1}\sub{#2}}}% #2-framing of #1\sub#2
\newcommand\Seifpair[3]{({#1},{#2})_{#3}} % pairing of #1 and #2 on #3
\newcommand\Seifsurf[1]{S({\diagram{#1}})}% Seifert surface gen. from data #1
\newcommand{\shoutfont}{\emph} % could be \textit, etc.
\newcommand{\shout}[1]{\shoutfont{#1}} % for REAL emphasis
\newcommand\simplepts[1]{\operatorname{simp}({#1})}% simplepoints of #1
\newcommand\sign[1]{\varepsilon({#1})} % sign (of a band, crossing, or whatever)
\newcommand\skel[2]{#1^{{\scriptscriptstyle({#2})}}} % #2-skeleton of #1
\newcommand{\speak}[1]{``#1''} % could be same as shout
\newcommand\sph{\Sigma} % sphere
\newcommand\sgn{\operatorname{sgn}} % signum
\newcommand\sing[1]{\operatorname{Sing}({#1})} % singular points of #1
\newcommand\singkth[2]{\operatorname{Sing}^{#1}({#2})} 
\newcommand\smoothloc[2]{\operatorname{sm}({#1};{#2})} % smoothing of #1 at #2
\newcommand\smooth[1]{\operatorname{sm}({#1})} % smoothing of #1
\newcommand\ssge{{\scriptscriptstyle\ge}}
\newcommand\ssle{{\scriptscriptstyle\le}}
\newcommand{\starx}{\thinspace{\lower .75ex \hbox {\text {\bxtwelve *}}}\thinspace }
\newcommand\stratum[2]{{\mathscr #1}_{#2}} % stratum named #1_#2
\newcommand\sub{\subset} 
\newcommand\subsets[2]{{\textstyle\binom{\textstyle #2}{\textstyle #1}}}% #1-subsets of #2
\newcommand\suchthat{\mathrel{\colon}} % before \mapsto
\newcommand\Suchthat{\mathrel{\colon}\linebreak[2]} % for set-building;
  %% \Suchthat could be |, depending on publisher's style

%%%%%%
\newcommand\supp[1]{\operatorname{supp}({#1})} % support of %1
\newcommand\surjection{\twoheadrightarrow}
\newcommand\sw{\operatorname{sw}} % Laufer's self-winding
\newcommand\symgroup[1]{\mathfrak{S}_#1} % symmetric group on #1 letters
\newcommand\sympower[2]{#1^#2/\symgroup{#2}} % #2th symmetric power of #1


\newcommand\tanbun[1]{T({#1})} % total space of the tangent bundle of #1
%\newcommand\tanbunmap[1]{\tau_{#1}} % tangent bundle map of #1
\newcommand\tanspace[2]{T_{#1}({#2})} % tangent space at #1 of #2
\newcommand\tb{\operatorname{tb}}  % Thurston-Bennequin invariant
\newcommand\TB{\operatorname{TB}}  % maximal Thurston-Bennequin invariant 
\newcommand\tframe[1]{\operatorname{tf({#1})}}% total framing of #1
\newcommand{\thru}{\nobreakdash--} % (requires amsmath!)
\newcommand\tlink[1]{\operatorname{tl({#1})}}% total linking of #1
\renewcommand\top[1]{\operatorname{top}({#1})} % top of #1 (a Seifert surface)
\newcommand\transpose[1]{{#1}^{\textsc{T}}} % transpose of (matrix) #1
\newcommand\transp[2]{({#1}\medspace{#2})} % transposition
\newcommand\transv[1]{\tau({#1})} % transverse arc of a 1-handle
\newcommand\tuple[3]{({#1}_{#2},\dots,{#1}_{#3})\/}%ordered tuple of #1s from #2 to #3
    \newcommand\parentuple[3]{({#1}({#2}),\dots,#1({#3}))\/}%
    %  ordered tuple of #1s from #2 to #3
\newcommand\type{\tau} % type (of a partition, etc.)
    \newcommand\ctype{\type^{c}} % ``connected type''
    \newcommand\typeof[1]{\type({#1})} % type of #1
\newcommand\Ts{\mathscr T}

\newcommand\utupsep[5]{\{{#1}_{#2} #4 #5 #4 {#1}_{#3}\}\/}
   %unordered tuple of #1s from #2 to #3, separated by #4, dotstyle #5
\newcommand\utuple[3]{\utupsep{#1}{#2}{#3}{,}{\dots}}
   \newcommand\untuple[2]{\utuple{#1}{1}{#2}}% unordered #2-tuple of #1s
\newcommand\ultuple[2]{\utupsep{#1}{1}{#2}{<}{\dotsm}}% "less-tuple"
\newcommand\underx[1]{{#1}_{\smallfrown}}%undercrossing at #1
\newcommand\Us{\mathscr U}
  \newcommand\spcheck{~\check\mathstrut} % instead of loading amsxtra
\newcommand\unclose[1]{#1\spcheck} % a braid whose closure is #1
\newcommand\Unorder[2]{U_{{#1},{#2}}}% "unordering map" of #2-tuples from #1
\newcommand\unorient[1]{|#1|} % the unoriented manifold underlying #1
\newcommand\usz{\mathaccent"707F{u}}%Uberschneidungszahl, of course!

\makeatletter
\mathchardef\Unfold@="1007 
 \newcommand\Unfold{\DOTSB\Unfold@\slimits@}% Neumann-Rudolph unfolding
\makeatother

\newcommand\valence[2]{\valfun{#2}({#1})} % valence of #1 in #2 
  \newcommand\valfun[1]{\operatorname{val}_{#1}}
\newcommand\variety[1]{\mathscr{V}_{#1}}% variety of zeroes of the function #1
\newcommand\Verts[1]{{\mathsf V}({#1})} % vertices of #1
\newcommand\vunknot{\mathbb{O}} % the vertical unknot

\newcommand\Weier[1]{{#1}_\bigtriangleup}% "Weierstrassification" of #1
   \newcommand\unWeier[1]{{#1}_\bigtriangledown}%"unWeierstrassification" of #1
\newcommand\wires[1]{\mathsf{W}({#1})} % wires of #1
\newcommand\Ws{\mathscr W}

\newcommand\Xs{\mathscr X} 
\newcommand{\Xge}[2]{{#1}_{\ge{#2}}}
\newcommand{\Xle}[2]{{#1}_{\le{#2}}}
\newcommand\Xend{X_{\mathrm{end}}} 

\newcommand\YBax[2]{\mathop{\llless}#1,#2\mathop{\gggtr}}% yangbaxter (tref.rel'n)
\newcommand\Ys{\mathscr Y}

\newcommand\Z{\mathbb Z}
\newcommand\zero{\mathbf{0}}



%%%% homemade `connected sum' symbols (take the place of \sharp, \natural):
\newcommand\overstrike[2]{{\setbox0\hbox{$#2$}\hbox to \wd0{\hss
                         ${#1}$\hss}\kern-\wd0\box0}}
\newcommand\onebar[2]{\hrule height#1ex width#2ex}
\newcommand\twobars[5]{\vcenter{\hrule height#1ex width#2ex
                               \vskip#3ex
                               \hrule height#4ex width#5ex}}
\newcommand\stroke[3]{\vrule height#1ex width#2ex depth#3ex}
\newcommand\connsum{\mathop{\raise.25ex\hbox{\overstrike\parallel=}}}
\newcommand\Connsum{\mathop{\displaystyle\raise.25ex\hbox{\overstrike\parallel=}}}
\newcommand\bdconnsum{\mathop{{}\hskip.3ex
                   \stroke{1.7}{.06}{-.13}
                   \twobars{.06}{.7}{.8}{.06}{.7}
                   \stroke{1.03}{.06}{.54}
                   \hskip.3ex{}}}
\newcommand\Bdconnsum{\bdconnsum}
%\newcommand\splitsum{\coprod}
\newcommand\splitsum{\sqcup}


%%%% plumbing:
     \font\bxtwelve=cmbx12      
\newcommand\plumb[1]{\mathop{\lower.75ex%
          \hbox{\text{\bxtwelve*}}}_{#1}} % plumb along #1
\def\topplumb#1{\mathop{{\overline\ast}\thinspace}_#1}
\def\botplumb#1{\mathop{{\underline\ast}\thinspace}_#1}
\def\PLUMB{\mathop{\displaystyle\ast}\nolimits}
\def\TOPPLUMB{\mathop{{\displaystyle\overline\ast}\thinspace}\nolimits}
\def\BOTPLUMB{\mathop{{\displaystyle\underline\ast}\thinspace}\nolimits}


     
%% for bibtex from AMS:
\def\cftil#1{\ifmmode\setbox7\hbox{$\accent"5E#1$}\else
\setbox7\hbox{\accent"5E#1}\penalty 10000\relax\fi\raise 1\ht7
\hbox{\lower1.15ex\hbox to 1\wd7{\hss\accent"7E\hss}}\penalty 10000
\hskip-1\wd7\penalty 10000\box7}
\def\cflex{\^} % as used in some MathSciNet MR citations
\def\cfudot#1{\cflex#1}

\font\manual=manfnt at 8pt
\font\tinymanual=manfnt at 6pt
\def\dbend{{\manual\char127}} % dangerous bend sign
\def\tinydbend{{\tinymanual\char127}} 
\def\danger{\protect%\reversemarginpar%
            \marginpar{$\genfrac{}{}{0pt}{}{\text{\dbend}}{\text{~}}$}}
\def\indanger#1{\hyperpage{#1}\danger}
\newcommand\bydefdanger[1]%
        {\danger\bydeffont{#1}\index{#1|indanger}}%could add \label{def:#1}
\newcommand\moredefdanger[1]{\danger\bydeffont{#1}}



